A Unifying Framework for Sparsity Constrained Optimization

In this paper, we consider the optimization problem of minimizing a continuously differentiable function subject to both convex constraints and sparsity constraints. By exploiting a mixed-integer reformulation from the literature, we define a necessary optimality condition based on a tailored neighborhood that allows to take into account potential changes of the support set. We then propose an algorithmic framework to tackle the considered class of problems and prove its convergence to points satisfying the newly introduced concept of stationarity. We further show that, by suitably choosing the neighborhood, other well-known optimality conditions from the literature can be recovered at the limit points of the sequence produced by the algorithm. Finally, we analyze the computational impact of the neighborhood size within our framework and in the comparison with some state-of-the-art algorithms, namely, the Penalty Decomposition method and the Greedy Sparse-Simplex method. The algorithms have been tested using a benchmark related to sparse logistic regression problems.

==> sections/neighborhoods_old.tex <==
The crucial point in the mixed-integer approach is choosing suitable discrete neighborhoods. First, note that when we deal with both continuous and integer variables, the usual notion of convergence to a point needs to be tweaked. In particular, we have the following definition.

\begin{definition}
A sequence $\{ (x^k, y^k) \}$ converges to a point $(\bar{x}, \bar{y})$ if for any $\epsilon > 0$ there exists an index $k_\epsilon$ such that for all $k \geq k_\epsilon$ we have that $y^k = \bar{y}$ and $\| x^k - \bar{x} \| < \epsilon$.
\end{definition}

To ensure convergence to meaningful points, we need a ``continuity" assumption on the discrete neighborhoods we explore.

\begin{assumption}
\label{asmp:discrete_neighborhood}
Let $\{ (x^k, y^k) \}$ be a sequence converging to $(\bar{x}, \bar{y})$. Then, for any $(\hat{x}, \hat{y}) \in \N(\bar{x}, \bar{y})$, there exists a sequence $\{ (\hat{x}^k, \hat{y}^k) \}$ converging to $(\hat{x}, \hat{y})$ such that $(\hat{x}^k, \hat{y}^k) \in \N(x^k, y^k)$.
\end{assumption}
The assumption above is a mild continuity assumption on the discrete neighborhoods and is equivalent to the lower semicontinuity of a point-to-set function as defined in \cite{Berge1963}. Next, we give an example of a possible discrete neighborhood.

\begin{example}
\label{ex:discrete_neighborhood}
Let $s=3$, $n=7$,
\[x=(2 1 3 0 0 0 0)^\top, \ y=(0 0 0 1 1 1 1)^\top. \]
First, we define $\N_s(x, y)$ as follows:
\begin{equation*}
\begin{array}{ccc}
(0 1 3 2 0 0 0)^\top, && (1 0 0 0 1 1 1)^\top,\\
(0 1 3 0 2 0 0)^\top, && (1 0 0 1 0 1 1)^\top,\\
&\vdots& \\
(2 1 0 0 0 0 3)^\top, && (0 0 1 1 1 1 0)^\top,\\
\end{array}
\end{equation*}
i.e., the set $\N_s(x, y)$ is defined by 12 points obtained by sequentially performing a swap, one at time, between zero and nonzero variables.
Then, we define $\N(x, y)$ as follows:

\begin{equation*}
\N(x, y) = \N_S(x, y) \cup \{ (x, y - e_j) \mid y - e_j \in \Y \} \cup \{ (x- x_j e_j, y + e_j ) \mid y + e_j \in \Y \}.
\end{equation*}
For example, if $s=2$, $n=3$,
\[x=(1 0 0)^\top, \ y=(0 1 1)^\top. \]
Then, $\N(x, y)$ contains the points
\begin{equation*}
\begin{array}{cc}
(1 0 0)^\top, & (0 0 1)^\top,\\
(1 0 0)^\top, & (0 1 0)^\top,\\
(0 0 0)^\top, & (1 1 1)^\top,\\
(0 1 0)^\top, & (1 0 1)^\top,\\
(0 0 1)^\top, & (1 1 0)^\top.\\
\end{array}
\end{equation*}
\end{example}

Now, a discrete neighborhood, by definition, is a set of feasible points. In the case when $X \subset \R^n$, swapping variables may result in points that are not feasible. For this reason, we initially consider an easier version of problem \cref{prob: mi_prob} where $\X = \R^n$.

\begin{proposition}
\label{prop:discrete_neighborhoods_no_X}
Let $\{(x^k, y^k)\}$ be a sequence converging to $(\bar{x}, \bar{y})$. Let $\N(\bar{x}, \bar{y})$ be the discrete neighborhood as defined in \cref{ex:discrete_neighborhood}. Then, $\N(\bar{x}, \bar{y})$ satisfies \cref{asmp:discrete_neighborhood}.
\end{proposition}

\begin{proof}
If $\{(x^k, y^k)\}$ converges to $(\bar{x}, \bar{y})$, then for any $\epsilon > 0$ there exists an index $k_\epsilon$ such that for all $k \geq k_\epsilon$ we have that $y^k = \bar{y}$ and $\| x^k - \bar{x} \| < \epsilon$. Let $(\hat{x}, \hat{y}) \in \N(\bar{x}, \bar{y})$.

First, suppose that $e^\top \bar{y} = e^\top \hat{y}$. Then, by definition, $(\hat{x}, \hat{y})$ is obtained by applying a permutation to $(\bar{x}, \bar{y})$. Formally, we can say that $(\hat{x}, \hat{y}) = p(\bar{x}, \bar{y})$, where $p: \R^{2n} \to \R^{2n}$ is the function that applies this permutation.

Let $\{(\hat{x}^k, \hat{y}^k)\}$ be the sequence such that $(\hat{x}^k, \hat{y}^k) = p(x^k, y^k)$ for all $k$. Note that $(\hat{x}^k, \hat{y}^k) \in \N(x^k, y^k)$ for all $k$.

Fix an $\epsilon > 0$. For $k \geq k_\epsilon$, we then have that $y^k = \bar{y}$, since $\{(x^k, y^k)\}$ converges to $(\bar{x}, \bar{y})$. This implies that $\hat{y}^k = \hat{y}$, by definition of $p$. Moreover, for $k \geq k_\epsilon$, we have that $\| \hat{x}^k - \hat{x} \| < \epsilon$, since $x^k$ is such that $\| x^k - \bar{x} \| < \epsilon$ and we have that $(\hat{x}^k, \hat{y}^k) = p(x^k, y^k)$ and $(\hat{x}, \hat{y}) = p(\bar{x}, \bar{y})$ (a permutation does not change distances). In other words, the sequence $\{ (\hat{x}^k, \hat{y}^k)\}$ converges to $(\hat{x}, \hat{y})$ and $(\hat{x}^k, \hat{y}^k) \in \N(x^k, y^k)$ for all $k$.

Suppose now that $\hat{y} = \bar{y} - e_j$, for some $j \in \{1,\ldots,n\}$. By definition of $\N(\bar{x}, \bar{y})$, we then have that $\hat{x} = \bar{x}$. For all $k$, let
$$\tilde{y}^k_i = \begin{cases}
\begin{array}{cl}
y^k_i & \text{if} \ i \ne j,\\
0 & \text{if} \ i = j,
\end{array}
\end{cases}$$
and let $\tilde{x}^k = x^k$. If $\tilde{y}^k \ne y^k$, then $(\tilde{x}^k, \tilde{y}^k) \in \N(x^k, y^k)$, and we define $(\hat{x}^k, \hat{y}^k) = (\tilde{x}^k, \tilde{y}^k)$. Otherwise, let $(\hat{x}^k, \hat{y}^k)$ be an arbitrary vector in $\N(x^k, y^k)$.
As in the previous case, $y^k = \bar{y}$ for all $k \geq k_\epsilon$, which implies that $\tilde{y}^k = \hat{y} \ne y^k$. This, in turn, yields that $\hat{y}^k = \hat{y}$ and $\hat{x}^k = x^k$ for all $k \geq k_\epsilon$. Then, $\norm{\hat{x}^k - \hat{x}} = \norm{x^k - \bar{x}} < \epsilon$, i.e., the sequence $\{ (\hat{x}^k, \hat{y}^k)\}$ converges to $(\hat{x}, \hat{y})$ and $(\hat{x}^k, \hat{y}^k) \in \N(x^k, y^k)$ for all $k$.

Finally, suppose that $\hat{y} = \bar{y} + e_j$, for some $j \in \{1,\ldots,n\}$. By definition of $\N(\bar{x}, \bar{y})$, we then have that $\hat{x} = \bar{x} - \bar{x}_j e_j$. Similarly to the previous case, for all $k$ we define
$$\tilde{y}^k_i = \begin{cases}
\begin{array}{cl}
y^k_i & \text{if} \ i \ne j,\\
1 & \text{if} \ i = j,
\end{array}
\end{cases}$$
and let $\tilde{x}^k = x^k - x^k_j e_j$. If $\tilde{y}^k \ne y^k$, then $(\tilde{x}^k, \tilde{y}^k) \in \N(x^k, y^k)$, and we define $(\hat{x}^k, \hat{y}^k) = (\tilde{x}^k, \tilde{y}^k)$. Otherwise, let $(\hat{x}^k, \hat{y}^k)$ be an arbitrary vector in $\N(x^k, y^k)$. Again, $y^k = \bar{y}$ for all $k \geq k_\epsilon$, which implies that $\tilde{y}^k = \hat{y} \ne y^k$. Therefore, $\hat{y}^k = \hat{y}$ and $\hat{x}^k = x^k - x^k_j e_j$ for all $k \geq k_\epsilon$. In other words, also recalling the definition of $\hat{x}$, we have that
\[ \hat{x}^k_i =
\begin{cases}
\begin{array}{cl}
x^k & i \ne j\\ 
0 & i = j \\
\end{array}
\end{cases},
\quad \hat{x}_i =
\begin{cases}
\begin{array}{cl}
\bar{x} & i \ne j\\ 
0 & i = j \\
\end{array}
\end{cases}.\]
Then, $\norm{\hat{x}^k - \hat{x}} \le \norm{x^k - \bar{x}} < \epsilon$, i.e., the sequence $\{ (\hat{x}^k, \hat{y}^k)\}$ converges to $(\hat{x}, \hat{y})$ and $(\hat{x}^k, \hat{y}^k) \in \N(x^k, y^k)$ for all $k$.
\end{proof}

To generalize the previous proposition to the case when $\X \subset \R^n$, we replace each $(\bar{x}, \bar{y}) \in \N(x,y)$ with the point $(\hat{x}, \hat{y})$, where $\hat{y} = \bar{y}$ and $\hat{x} = \Pi_{\X(\hat{y})}(\bar{x})$. In other words, first we ``change" $(x,y)$ as in \cref{ex:discrete_neighborhood}, then we project the $x$ part onto $\X$ with our custom projection operator. In the following, we will refer to this new discrete neighborhood with $\N_C(x,y)$.

\begin{proposition}
\label{prop:discrete_neighborhoods_X}
Let $\{(x^k, y^k)\}$ be a sequence converging to $(\bar{x}, \bar{y})$. Then, $\N_C(\bar{x}, \bar{y})$ satisfies \cref{asmp:discrete_neighborhood}.
\end{proposition}
\begin{proof}
Let $(\hat{x}_C, \hat{y}_C) \in \N_C(\bar{x}, \bar{y})$. By definition, there exist a point $(\hat{x},\hat{y}) \in N(\bar{x}, \bar{y})$ such that $\hat{y}_C = \hat{y}$ and $\hat{x}_C = \Pi_{\X(\hat{y})}(\hat{x})$. Consider the sequence $\{(\hat{x}^k, \hat{y}^k)\}$ as defined in \cref{prop:discrete_neighborhoods_no_X}, and define the sequence $\{ (\hat{x}^k_C, \hat{y}^k_C) \}$ where $\hat{y}^k_C = \hat{y}^k$ and $\hat{x}^k_C = \Pi_{\X(\hat{y}^k)}(\hat{x}^k)$ for all $k$. By definition, $(\hat{x}^k_C, \hat{y}^k_C) \in \N_C(x^k, y^k)$ for all $k$.

By \cref{prop:discrete_neighborhoods_no_X}, we have that $\hat{x}^k \to \hat{x}$, and $\hat{y}^k_C = \hat{y}^k = \hat{y}$ for $k$ sufficiently large. Since $\Pi_{\X(\hat{y})}$ is continuous, this entails that
$\Pi_{\X(\hat{y})}(\hat{x}^k) \to \Pi_{\X(\hat{y})}(\hat{x})$, which is saying that $\hat{x}^k_C \to \hat{x}_C$. In other words, the sequence $\{(\hat{x}^k_C, \hat{y}^k_C)\}$ converges to $(\hat{x}_C, \hat{y}_C)$ and the claim holds.
\end{proof}
